Entropy-Regularized Reinforcement Learning for Regime-Switching Stochastic Control: A Study on Distributional Classes

We study entropy-regularized reinforcement learning for finite-horizon stochastic control with Markov regime switching, emphasizing the benefits of distributional structure priors. The action domain and the action dependence of the exploratory Hamiltonian identify explicit policy families, including Gaussian, Gamma, Beta, Dirichlet, Weibull, Pareto, and log-normal distributions. These analytical relations guide a structure-informed continuous-time $q$-learning method: the policy respects the prescribed action support, shares parameters with a normalized $q$-function, and incorporates known distributional parameters before learning. This construction avoids numerical action-space normalization and reduces the number of parameters requiring estimation. In a consumption-investment application, finiteness of the optimized HJB Hamiltonian implies positive marginal value and strictly negative wealth curvature for any smooth finite-valued solution, yielding independent Gamma consumption and Gaussian investment policies. A logarithmic terminal-utility benchmark permits independent assessment of learning accuracy and discretization error. Across ten paired random seeds, fixing the known consumption-shape parameter reduces the mean number of updates required to reach a specified policy-error threshold by 12.6\%, with comparable final accuracy. A separate mesh study identifies first-order discretization error. These results illustrate how distributional information can simplify policy learning while retaining flexibility in the unknown parameter functions.

==> numerics/learning_figure.tex <==
\begin{figure}[tbp]
\centering
\begin{tikzpicture}
\begin{groupplot}[group style={group size=2 by 1,horizontal sep=1.25cm},width=0.45\textwidth,height=5.1cm,xlabel={Updates},ymode=log,grid=major,legend style={font=\scriptsize,at={(0.98,0.98)},anchor=north east},tick label style={font=\scriptsize},label style={font=\small}]
\nextgroupplot[ylabel={$E_{\mathrm{KL}}$}]
\addplot[name path=fixedupper,draw=none,forget plot] coordinates {(0,0.62903128) (100,0.69126117) (200,0.64944845) (300,0.44537473) (400,0.31570639) (500,0.23733513) (600,0.16998906) (700,0.1200431) (800,0.078880955) (900,0.049215744) (1000,0.028228832) (1100,0.017312051) (1200,0.012207988) (1300,0.010357138) (1400,0.0087464785) (1500,0.0070255218) (1600,0.0055486064) (1700,0.0038783021) (1800,0.0029363184) (1900,0.0020697353) (2000,0.0017424771) (2100,0.0011888723) (2200,0.0011406984) (2300,0.0010256276) (2400,0.0007030307) (2500,0.00093351228) (2600,0.00069936574) (2700,0.00095208309) (2800,0.00086861363) (2900,0.00072451658) (3000,0.00086676235) (3100,0.00063754906) (3200,0.00098373327) (3300,0.00072615503) (3400,0.0006597347) (3500,0.00061843248) (3600,0.0007676253) (3700,0.00081719279) (3800,0.00063943628) (3900,0.00083957161) (4000,0.00071226722) (4100,0.00080548839) (4200,0.00064907655) (4300,0.00091865348) (4400,0.0009430715) (4500,0.00090883883) (4600,0.00061116802) (4700,0.00099330206) (4800,0.00056098487) (4900,0.00084842671) (5000,0.00071906889)};
\addplot[name path=fixedlower,draw=none,forget plot] coordinates {(0,0.62903128) (100,0.6719091) (200,0.59749882) (300,0.42425093) (400,0.30040886) (500,0.22531262) (600,0.16103637) (700,0.10884673) (800,0.070369173) (900,0.043883507) (1000,0.025287994) (1100,0.015352148) (1200,0.011404017) (1300,0.0094533425) (1400,0.0079545229) (1500,0.0063581168) (1600,0.0047606964) (1700,0.0035749735) (1800,0.0024079839) (1900,0.0017413311) (2000,0.0012901817) (2100,0.00091881048) (2200,0.00076072562) (2300,0.00046460887) (2400,0.00048341562) (2500,0.00038506426) (2600,0.00034303494) (2700,0.00022224155) (2800,0.00029924893) (2900,0.00030367087) (3000,0.00027215027) (3100,0.00021648182) (3200,0.00015509274) (3300,0.00028619786) (3400,0.00017613393) (3500,0.00037024787) (3600,0.00041185384) (3700,0.00013135683) (3800,0.00022314102) (3900,0.00017726206) (4000,0.00012358144) (4100,0.00024518396) (4200,0.00013022362) (4300,0.00017189219) (4400,0.00018655606) (4500,0.00024183689) (4600,0.00021924771) (4700,0.00014788545) (4800,0.00031495073) (4900,0.00016918922) (5000,0.0002333224)};
\addplot[blue!70!black,fill opacity=0.12,forget plot] fill between[of=fixedupper and fixedlower];
\addplot[blue!70!black,thick] coordinates {(0,0.62903128) (100,0.68158514) (200,0.62347363) (300,0.43481283) (400,0.30805763) (500,0.23132388) (600,0.16551271) (700,0.11444491) (800,0.074625064) (900,0.046549626) (1000,0.026758413) (1100,0.0163321) (1200,0.011806002) (1300,0.0099052404) (1400,0.0083505007) (1500,0.0066918193) (1600,0.0051546514) (1700,0.0037266378) (1800,0.0026721512) (1900,0.0019055332) (2000,0.0015163294) (2100,0.0010538414) (2200,0.00095071202) (2300,0.00074511822) (2400,0.00059322316) (2500,0.00065928827) (2600,0.00052120034) (2700,0.00058716232) (2800,0.00058393128) (2900,0.00051409372) (3000,0.00056945631) (3100,0.00042701544) (3200,0.00056941301) (3300,0.00050617645) (3400,0.00041793431) (3500,0.00049434018) (3600,0.00058973957) (3700,0.00047427481) (3800,0.00043128865) (3900,0.00050841683) (4000,0.00041792433) (4100,0.00052533618) (4200,0.00038965008) (4300,0.00054527283) (4400,0.00056481378) (4500,0.00057533786) (4600,0.00041520787) (4700,0.00057059376) (4800,0.0004379678) (4900,0.00050880796) (5000,0.00047619565)};
\addlegendentry{Fixed known shape}
\addplot[name path=freeupper,draw=none,forget plot] coordinates {(0,0.62903128) (100,0.68262411) (200,0.53488056) (300,0.30270726) (400,0.16287028) (500,0.10085995) (600,0.081312151) (700,0.066210426) (800,0.052389454) (900,0.04143541) (1000,0.032831555) (1100,0.025923809) (1200,0.020254172) (1300,0.016261247) (1400,0.012686176) (1500,0.0099638256) (1600,0.0078021101) (1700,0.0060201393) (1800,0.0047817079) (1900,0.0036122624) (2000,0.0028785627) (2100,0.0023197482) (2200,0.0019089971) (2300,0.0016556085) (2400,0.0012093683) (2500,0.0012415531) (2600,0.00097679425) (2700,0.0011494167) (2800,0.00088929965) (2900,0.00078554588) (3000,0.00090369284) (3100,0.00069261958) (3200,0.00085154045) (3300,0.00079784937) (3400,0.00067533021) (3500,0.00054657036) (3600,0.00070103865) (3700,0.00070216412) (3800,0.00058217072) (3900,0.00067726964) (4000,0.0006597141) (4100,0.00077700635) (4200,0.00073690067) (4300,0.00081292912) (4400,0.00083492261) (4500,0.00081841564) (4600,0.00064544834) (4700,0.0010092017) (4800,0.00052569674) (4900,0.00078805754) (5000,0.00082684605)};
\addplot[name path=freelower,draw=none,forget plot] coordinates {(0,0.62903128) (100,0.66759209) (200,0.50395683) (300,0.25289972) (400,0.13120944) (500,0.095871916) (600,0.079262603) (700,0.061970585) (800,0.049795801) (900,0.03918609) (1000,0.031514979) (1100,0.024388751) (1200,0.019226002) (1300,0.015091675) (1400,0.011887916) (1500,0.0092921877) (1600,0.0073414682) (1700,0.0056008356) (1800,0.004256202) (1900,0.0032794959) (2000,0.0025890637) (2100,0.0019424707) (2200,0.0015622365) (2300,0.0011090907) (2400,0.00092152824) (2500,0.00084896078) (2600,0.00059225048) (2700,0.00039987614) (2800,0.00050980251) (2900,0.00045634019) (3000,0.00036530802) (3100,0.00027820758) (3200,0.00024474611) (3300,0.0002796854) (3400,0.00023893983) (3500,0.00038296978) (3600,0.00036300844) (3700,0.0002078577) (3800,0.00020684521) (3900,0.00023445451) (4000,0.00014753225) (4100,0.00017932257) (4200,0.00012087187) (4300,0.00021685372) (4400,0.00019729956) (4500,0.00024552328) (4600,0.00025601492) (4700,0.00019217651) (4800,0.00032068989) (4900,0.00021054259) (5000,0.00025241042)};
\addplot[orange!85!black,fill opacity=0.12,forget plot] fill between[of=freeupper and freelower];
\addplot[orange!85!black,thick] coordinates {(0,0.62903128) (100,0.6751081) (200,0.51941869) (300,0.27780349) (400,0.14703986) (500,0.098365933) (600,0.080287377) (700,0.064090506) (800,0.051092628) (900,0.04031075) (1000,0.032173267) (1100,0.02515628) (1200,0.019740087) (1300,0.015676461) (1400,0.012287046) (1500,0.0096280067) (1600,0.0075717892) (1700,0.0058104875) (1800,0.004518955) (1900,0.0034458792) (2000,0.0027338132) (2100,0.0021311095) (2200,0.0017356168) (2300,0.0013823496) (2400,0.0010654483) (2500,0.0010452569) (2600,0.00078452237) (2700,0.00077464642) (2800,0.00069955108) (2900,0.00062094303) (3000,0.00063450043) (3100,0.00048541358) (3200,0.00054814328) (3300,0.00053876739) (3400,0.00045713502) (3500,0.00046477007) (3600,0.00053202355) (3700,0.00045501091) (3800,0.00039450796) (3900,0.00045586207) (4000,0.00040362317) (4100,0.00047816446) (4200,0.00042888627) (4300,0.00051489142) (4400,0.00051611108) (4500,0.00053196946) (4600,0.00045073163) (4700,0.00060068909) (4800,0.00042319332) (4900,0.00049930006) (5000,0.00053962823)};
\addlegendentry{Learned shape}
\nextgroupplot[ylabel={$E_V$}]
\addplot[name path=fixedupper,draw=none,forget plot] coordinates {(0,0.60861946) (100,0.36211705) (200,0.25411116) (300,0.18359986) (400,0.14182853) (500,0.11745254) (600,0.10194436) (700,0.089737956) (800,0.079698927) (900,0.070504368) (1000,0.062409935) (1100,0.054800286) (1200,0.048057479) (1300,0.042653918) (1400,0.036677236) (1500,0.031879129) (1600,0.027986456) (1700,0.024276989) (1800,0.020742684) (1900,0.017020044) (2000,0.016257755) (2100,0.013240235) (2200,0.011375968) (2300,0.011390834) (2400,0.0089407449) (2500,0.0087052254) (2600,0.0070596206) (2700,0.007504956) (2800,0.0072172227) (2900,0.0067609972) (3000,0.00718726) (3100,0.0055106335) (3200,0.0060445877) (3300,0.0055331132) (3400,0.0053262875) (3500,0.005260552) (3600,0.0070669502) (3700,0.0051433912) (3800,0.0043058124) (3900,0.0066779221) (4000,0.005096375) (4100,0.0053692948) (4200,0.0056358705) (4300,0.005598931) (4400,0.00567838) (4500,0.0060252394) (4600,0.0044123967) (4700,0.0063223436) (4800,0.0047376671) (4900,0.0056530611) (5000,0.0052870404)};
\addplot[name path=fixedlower,draw=none,forget plot] coordinates {(0,0.60861946) (100,0.35917689) (200,0.25161962) (300,0.18126558) (400,0.1404676) (500,0.1156346) (600,0.10015704) (700,0.08769109) (800,0.078221347) (900,0.068778766) (1000,0.06080302) (1100,0.053030126) (1200,0.046795966) (1300,0.040627697) (1400,0.034443188) (1500,0.029865984) (1600,0.026159511) (1700,0.021844681) (1800,0.018742036) (1900,0.015388765) (2000,0.013529031) (2100,0.01092692) (2200,0.0093574679) (2300,0.0080177727) (2400,0.0064244951) (2500,0.0064637356) (2600,0.0046045755) (2700,0.0046509329) (2800,0.0039374271) (2900,0.0032969818) (3000,0.0039300368) (3100,0.003287627) (3200,0.0028001854) (3300,0.0031612725) (3400,0.0020522667) (3500,0.0024537697) (3600,0.0027429097) (3700,0.0024686381) (3800,0.001940316) (3900,0.0020165083) (4000,0.0024148012) (4100,0.0025791713) (4200,0.0020567467) (4300,0.0027335528) (4400,0.0026491981) (4500,0.0027782466) (4600,0.0027753333) (4700,0.0016651528) (4800,0.0019850579) (4900,0.0032537498) (5000,0.0029446459)};
\addplot[blue!70!black,fill opacity=0.12,forget plot] fill between[of=fixedupper and fixedlower];
\addplot[blue!70!black,thick] coordinates {(0,0.60861946) (100,0.36064697) (200,0.25286539) (300,0.18243272) (400,0.14114807) (500,0.11654357) (600,0.1010507) (700,0.088714523) (800,0.078960137) (900,0.069641567) (1000,0.061606477) (1100,0.053915206) (1200,0.047426723) (1300,0.041640807) (1400,0.035560212) (1500,0.030872557) (1600,0.027072984) (1700,0.023060835) (1800,0.01974236) (1900,0.016204405) (2000,0.014893393) (2100,0.012083578) (2200,0.010366718) (2300,0.0097043031) (2400,0.00768262) (2500,0.0075844805) (2600,0.0058320981) (2700,0.0060779444) (2800,0.0055773249) (2900,0.0050289895) (3000,0.0055586484) (3100,0.0043991302) (3200,0.0044223865) (3300,0.0043471928) (3400,0.0036892771) (3500,0.0038571609) (3600,0.0049049299) (3700,0.0038060146) (3800,0.0031230642) (3900,0.0043472152) (4000,0.0037555881) (4100,0.0039742331) (4200,0.0038463086) (4300,0.0041662419) (4400,0.004163789) (4500,0.004401743) (4600,0.003593865) (4700,0.0039937482) (4800,0.0033613625) (4900,0.0044534055) (5000,0.0041158431)};
\addlegendentry{Fixed known shape}
\addplot[name path=freeupper,draw=none,forget plot] coordinates {(0,0.60861946) (100,0.36726642) (200,0.25056516) (300,0.17995988) (400,0.14065996) (500,0.11811374) (600,0.10332572) (700,0.091462857) (800,0.081645802) (900,0.07248579) (1000,0.064428391) (1100,0.05701546) (1200,0.050548462) (1300,0.045357362) (1400,0.039599223) (1500,0.035110133) (1600,0.031436799) (1700,0.027813023) (1800,0.024357518) (1900,0.020626705) (2000,0.019678731) (2100,0.016493572) (2200,0.01441082) (2300,0.014106964) (2400,0.011531778) (2500,0.010865813) (2600,0.0090307463) (2700,0.0090742043) (2800,0.0087215811) (2900,0.0079056623) (3000,0.0081538106) (3100,0.0065142107) (3200,0.0067518808) (3300,0.0061346821) (3400,0.0057600064) (3500,0.0058065419) (3600,0.0073860145) (3700,0.0054330265) (3800,0.0045125639) (3900,0.006974216) (4000,0.0051322725) (4100,0.0053472975) (4200,0.0055982943) (4300,0.0056659079) (4400,0.0056250688) (4500,0.0060553159) (4600,0.0044231844) (4700,0.0063283568) (4800,0.0047214468) (4900,0.0055769024) (5000,0.0053098433)};
\addplot[name path=freelower,draw=none,forget plot] coordinates {(0,0.60861946) (100,0.3652399) (200,0.24896327) (300,0.1783841) (400,0.13967191) (500,0.11620756) (600,0.10161289) (700,0.089647816) (800,0.080238795) (900,0.070916218) (1000,0.062978813) (1100,0.055335126) (1200,0.049240758) (1300,0.043393218) (1400,0.03748048) (1500,0.033228403) (1600,0.029648522) (1700,0.025439159) (1800,0.022362595) (1900,0.018854536) (2000,0.016922823) (2100,0.014207557) (2200,0.012212821) (2300,0.010785502) (2400,0.0088789404) (2500,0.0085508524) (2600,0.0063211361) (2700,0.0062576221) (2800,0.0052841974) (2900,0.0042245007) (3000,0.004999102) (3100,0.0040434088) (3200,0.0034938193) (3300,0.0037668711) (3400,0.0025776816) (3500,0.0030401328) (3600,0.003110797) (3700,0.002832913) (3800,0.0022098662) (3900,0.0021853995) (4000,0.0025774521) (4100,0.002666091) (4200,0.002272533) (4300,0.0028615746) (4400,0.002778265) (4500,0.002801905) (4600,0.0030519742) (4700,0.0016995353) (4800,0.0020852749) (4900,0.0032792547) (5000,0.0030435576)};
\addplot[orange!85!black,fill opacity=0.12,forget plot] fill between[of=freeupper and freelower];
\addplot[orange!85!black,thick] coordinates {(0,0.60861946) (100,0.36625316) (200,0.24976421) (300,0.17917199) (400,0.14016593) (500,0.11716065) (600,0.10246931) (700,0.090555337) (800,0.080942298) (900,0.071701004) (1000,0.063703602) (1100,0.056175293) (1200,0.04989461) (1300,0.04437529) (1400,0.038539852) (1500,0.034169268) (1600,0.03054266) (1700,0.026626091) (1800,0.023360057) (1900,0.01974062) (2000,0.018300777) (2100,0.015350565) (2200,0.01331182) (2300,0.012446233) (2400,0.010205359) (2500,0.0097083328) (2600,0.0076759412) (2700,0.0076659132) (2800,0.0070028893) (2900,0.0060650815) (3000,0.0065764563) (3100,0.0052788098) (3200,0.00512285) (3300,0.0049507766) (3400,0.004168844) (3500,0.0044233373) (3600,0.0052484058) (3700,0.0041329697) (3800,0.0033612151) (3900,0.0045798077) (4000,0.0038548623) (4100,0.0040066943) (4200,0.0039354136) (4300,0.0042637413) (4400,0.0042016669) (4500,0.0044286104) (4600,0.0037375793) (4700,0.004013946) (4800,0.0034033609) (4900,0.0044280785) (5000,0.0041767005)};
\addlegendentry{Learned shape}
\end{groupplot}
\end{tikzpicture}
\caption{Learning curves over ten paired seeds. Solid curves show the arithmetic mean; shaded bands show one sample standard deviation. Each update uses 1,024 antithetic pairs, or 2,048 observed transitions.}
\label{fig:learning-curves}
\end{figure}

==> numerics/policy_figure.tex <==
\begin{figure}[tbp]
\centering
\begin{tikzpicture}
\begin{groupplot}[group style={group size=2 by 1,horizontal sep=1.25cm},width=0.45\textwidth,height=5cm,xlabel={$t$},grid=major,legend style={font=\scriptsize,at={(0.02,0.98)},anchor=north west},tick label style={font=\scriptsize},label style={font=\small}]
\nextgroupplot[ylabel={Mean consumption / wealth}]
\addplot[black,thick] coordinates {(0,0.54277005) (0.05,0.55662689) (0.1,0.57124414) (0.15,0.5866861) (0.2,0.60302454) (0.25,0.62033978) (0.3,0.63872205) (0.35,0.65827305) (0.4,0.67910782) (0.45,0.701357) (0.5,0.72516961) (0.55,0.75071634) (0.6,0.77819366) (0.65,0.8078289) (0.7,0.83988653) (0.75,0.8746761) (0.8,0.91256222) (0.85,0.9539774) (0.9,0.99943868) (0.95,1.0495692) (1,1.1051271)};
\addlegendentry{Benchmark}
\addplot[blue!70!black,thick,dashed] coordinates {(0,0.54472705) (0.05,0.5589881) (0.1,0.57390434) (0.15,0.58955964) (0.2,0.60604698) (0.25,0.62346916) (0.3,0.64193975) (0.35,0.66158405) (0.4,0.68254043) (0.45,0.70496181) (0.5,0.72901747) (0.55,0.75489517) (0.6,0.78280369) (0.65,0.81297582) (0.7,0.84567191) (0.75,0.88118402) (0.8,0.91984095) (0.85,0.96201406) (0.9,1.0081243) (0.95,1.0586506) (1,1.1141398)};
\addlegendentry{Learned, seed mean}
\nextgroupplot[ylabel={Portfolio standard deviation}]
\addplot[blue!70!black,thick] coordinates {(0,1.1106612) (0.05,1.1260281) (0.1,1.1420138) (0.15,1.1586616) (0.2,1.176019) (0.25,1.1941384) (0.3,1.2130779) (0.35,1.232902) (0.4,1.2536825) (0.45,1.2754995) (0.5,1.2984433) (0.55,1.322615) (0.6,1.3481293) (0.65,1.3751165) (0.7,1.4037252) (0.75,1.4341259) (0.8,1.4665155) (0.85,1.5011223) (0.9,1.5382136) (0.95,1.5781036) (1,1.6211656)};
\addlegendentry{Benchmark, regime 1}
\addplot[blue!70!black,thick,dashed] coordinates {(0,1.112677) (0.05,1.1277083) (0.1,1.1434589) (0.15,1.1599775) (0.2,1.1773166) (0.25,1.195532) (0.3,1.2146832) (0.35,1.2348339) (0.4,1.2560519) (0.45,1.2784095) (0.5,1.301984) (0.55,1.3268582) (0.6,1.3531204) (0.65,1.3808654) (0.7,1.4101949) (0.75,1.4412181) (0.8,1.4740527) (0.85,1.5088256) (0.9,1.5456738) (0.95,1.5847456) (1,1.6262019)};
\addlegendentry{Learned, regime 1}
\addplot[orange!85!black,thick] coordinates {(0,0.63466354) (0.05,0.64344461) (0.1,0.65257931) (0.15,0.66209233) (0.2,0.67201083) (0.25,0.68236478) (0.3,0.69318737) (0.35,0.70451542) (0.4,0.71638998) (0.45,0.72885688) (0.5,0.74196758) (0.55,0.75577999) (0.6,0.77035962) (0.65,0.78578088) (0.7,0.8021287) (0.75,0.81950054) (0.8,0.83800885) (0.85,0.8577842) (0.9,0.87897918) (0.95,0.90177348) (1,0.92638031)};
\addlegendentry{Benchmark, regime 2}
\addplot[orange!85!black,thick,dashed] coordinates {(0,0.63563692) (0.05,0.64491876) (0.1,0.65443302) (0.15,0.66422243) (0.2,0.67433242) (0.25,0.68481128) (0.3,0.69571033) (0.35,0.70708415) (0.4,0.71899079) (0.45,0.73149211) (0.5,0.74465415) (0.55,0.7585475) (0.6,0.77324781) (0.65,0.78883634) (0.7,0.80540058) (0.75,0.82303503) (0.8,0.84184195) (0.85,0.86193238) (0.9,0.8834272) (0.95,0.90645837) (1,0.93117033)};
\addlegendentry{Learned, regime 2}
\end{groupplot}
\end{tikzpicture}
\caption{Policy moments for the logarithmic benchmark and the fixed-shape learner after 5,000 updates, averaged over ten seeds. Consumption divided by wealth is independent of the current regime in this particular benchmark.}
\label{fig:policy-moments}
\end{figure}
